TWIST: Teleoperated Whole-Body Imitation System

Teleoperating humanoid robots in a whole-body manner marks a fundamental step toward developing general-purpose robotic intelligence, with human motion providing an ideal interface for controlling all degrees of freedom. Yet, most current humanoid teleoperation systems fall short of enabling coordinated whole-body behavior, typically limiting themselves to isolated locomotion or manipulation tasks. We present the Teleoperated Whole-Body Imitation System (TWIST), a system for humanoid teleoperation through whole-body motion imitation. We first generate reference motion clips by retargeting human motion capture data to the humanoid robot. We then develop a robust, adaptive, and responsive whole-body controller using a combination of reinforcement learning and behavior cloning (RL+BC). Through systematic analysis, we demonstrate how incorporating privileged future motion frames and real-world motion capture (MoCap) data improves tracking accuracy. TWIST enables real-world humanoid robots to achieve unprecedented, versatile, and coordinated whole-body motor skills--spanning whole-body manipulation, legged manipulation, locomotion, and expressive movement--using a single unified neural network controller. Our project website: https://humanoid-teleop.github.io

==> tables/reward_expression.tex <==
% target keybody positions & $\exp(-\lVert \mathbf{p}_{\text{keybody}} - \mathbf{p}_{\text{keybody}}^{\text{tg}} \rVert^2)$ \\
% target joint positions & $\exp(-\lVert \mathbf{q} - \mathbf{q}^{\text{tg}} \rVert^2)$ \\
% target joint velocities & $\exp(-\lVert \mathbf{\dot{q}} - \mathbf{\dot{q}}^{\text{tg}} \rVert^2)$ \\
% target root pose & $\exp(-\lVert [r, p] - [r^{\text{tg}}, p^{\text{tg}}] \rVert^2 - |h-h^{\text{gt}}|^2)$\\
% target root velocity & $\exp(-\lVert \mathbf{v}-\mathbf{v}^{\text{gt}} \rVert^2)$ \\
% feet contact & $-(F_{\text{feet}} > 350)$ \\
% feet slipping & $-\lVert \mathbf{v}_{\text{feet}} \cdot \mathbf{1}[F_{\text{feet}} > 1] \rVert$ \\
% joint velocities & $-\lVert \dot{\mathbf{q}} \rVert$ \\
% joint acceleration & $-\lVert \ddot{\mathbf{q}} \rVert$ \\
% action rate & $-\lVert \mathbf{a}_{t} - \mathbf{a}_{t-1} \rVert$ \\
% feet air time & $ \min (t_{\text{air time}} - 0.25, 0)$ 
